Dominant Shuffle: A Simple Yet Powerful Data Augmentation for Time-series Prediction

Recent studies have suggested frequency-domain Data augmentation (DA) is effec tive for time series prediction. Existing frequency-domain augmentations disturb the original data with various full-spectrum noises, leading to excess domain gap between augmented and original data. Although impressive performance has been achieved in certain cases, frequency-domain DA has yet to be generalized to time series prediction datasets. In this paper, we found that frequency-domain augmentations can be significantly improved by two modifications that limit the perturbations. First, we found that limiting the perturbation to only dominant frequencies significantly outperforms full-spectrum perturbations. Dominant fre quencies represent the main periodicity and trends of the signal and are more important than other frequencies. Second, we found that simply shuffling the dominant frequency components is superior over sophisticated designed random perturbations. Shuffle rearranges the original components (magnitudes and phases) and limits the external noise. With these two modifications, we proposed dominant shuffle, a simple yet effective data augmentation for time series prediction. Our method is very simple yet powerful and can be implemented with just a few lines of code. Extensive experiments with eight datasets and six popular time series models demonstrate that our method consistently improves the baseline performance under various settings and significantly outperforms other DA methods. Code can be accessed at https://kaizhao.net/time-series.

==> abstract2.tex <==
Data augmentation (DA)
generates new samples by perturbing
existing data.
%
It's an efficient way to expanding the training set for various deep learning tasks.
%
Recent studies have suggested perturbing 
both the data and labels in the frequency domain 
to enhance the coherence between data and labels
for time series prediction.
%
However, existing frequency-domain DA methods
perturb the entire spectrum without differentiating 
frequency components.
%
And the perturbation operations either introduce new or eliminate
existing frequency components,
leading to inconsistency between augmented and original data distributions and
suboptimal performance.
%
Dominant frequencies with higher magnitudes
have been proven to  represent the main patterns and trends in the time series,
while other frequency components correspond
to noise or insignificant variations.
%
Perturbing only the dominant frequencies enriches the main trends and
reduces noisy information in a dataset.
%
In this paper, we proposed \emph{Dominant Shuffle}, a simple yet effective
frequency domain DA method that shuffles
dominant frequency components with the largest magnitudes.
%
Compared to full-spectrum randomization,
dominant shuffle enhances the \emph{coherence} without compromising diversity, 
leading to significantly better performance.
%
Extensive experiments with eight datasets 
and six popular time series models
demonstrate that
our method consistently improves 
the baseline performance under various settings
and significantly outperforms other DA methods.
%
Our method is intuitive, simple, and effective, which can be implemented
with a few lines of code.

==> tables/ablate_all.tex <==

&  & & \multicolumn{4}{c}{ETTh1} & \multicolumn{4}{c}{ETTm2} & \multicolumn{4}{c}{Weather} & \multicolumn{4}{c}{Exchange Rate} \\
& & & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 \\
\hline
\multirow{8}{*}{\rotatebox{90}{AutoFormer~\cite{wu2021autoformer}}} & \multirow{2}{*}{Msk} 
& full & 0.424 & 0.468 & \best{0.485} & \best{0.474} & 0.217 & \best{0.267} & 0.347 & 0.451 & 0.245 & 0.290 & 0.340 & 0.392 & 
0.142 & 0.410 & 0.471 & \best{0.778} \\
& & dom & \best{0.418} & \best{0.443} & 0.496 & 0.501
& \best{0.214} & 0.272 & \best{0.331} & \best{0.429} & \best{0.210} & \best{0.289} & \best{0.339} & \best{0.384} & \best{0.139} & \best{0.295} & \best{0.421} & 1.145  \\
\cdashline{2-18}
& \multirow{2}{*}{Nois} & full &0.437 &0.452&\best{0.492}& \best{0.477}& 0.235&	0.291&	0.375&	\best{0.478} &0.27 &0.334 &0.351 &0.429 &\best{0.142} &\best{0.309} &0.462 &1.123\\
& & dom & \best{0.432} &\best{0.451}& 0.501& 0.482& \best{0.223}	&\best{0.286}&	\best{0.355}&0.510&	\best{0.256}&
\best{0.302}	&\best{0.337}&	\best{0.399}	&0.156&	0.331&	\best{0.452}	&\best{0.914}\\
\cdashline{2-18}
& \multirow{2}{*}{Rnd} 
& full & 0.454 & 0.466 & 0.486 & \best{0.511} & 0.217 & \best{0.269} & \best{0.322} & \best{0.418} & 0.266 & 0.306 & 0.341 & 0.414 & 0.145 & \best{0.262} & 0.596 & 1.167 \\
& & dom & \best{0.451} & \best{0.440} & \best{0.484} & 0.552 & \best{0.212} & 0.276 & 0.333 & 0.464 & \best{0.248} & \best{0.284} & \best{0.337} & \best{0.410} & \best{0.141} & 0.297 & \best{0.577} & \best{0.985} \\
\cdashline{2-18}
& \multirow{2}{*}{Shuf} 
& full &  0.456 & 0.466 &  0.502 & 0.499  &  0.211&0.269  &0.332   & 0.450 &  0.262&0.284  &0.334  & \best{0.379} & 0.145 & 0.304 &0.438  & 0.796\\
& & dom & \best{0.409} & \best{0.436} &  \best{0.458} &  \best{0.486} & \best{0.210} & \best{0.266} & \best{0.329}  & \best{0.429} & \best{0.214} & \best{0.273} & \best{0.327} & 0.383 & \best{0.136} & \best{0.243} & \best{0.418} & \best{0.695} \\
\hline
\multirow{8}{*}{\rotatebox{90}{MICN~\cite{wang2023micn}}} & \multirow{2}{*}{Msk} & full & 0.381 & 0.424 & 0.460 & \best{0.543} & 0.184 & \best{0.265} & 0.353 & 0.510 & 0.190 & \best{0.236} & \best{0.281} & 0.345 & \best{0.085} & 0.173 & 0.339 & 0.847 \\
& & dom & \best{0.377} & \best{0.421} & \best{0.454} & 
\best{0.543} & \best{0.175} & 0.268 & \best{0.337} & \best{0.498} & \best{0.178} & 0.239 & 0.283 & \best{0.342} & 0.087 & \best{0.170} & \best{0.307} & \best{0.682} \\
\cdashline{2-18}
& \multirow{2}{*}{Nois} & full &\best{0.392}	&0.436	&0.491&	0.556& 0.203&	\best{0.298}&	0.372	&0.619&\best{0.192}&	0.239&	0.292	&\best{0.343}	&\best{0.085}	&0.179	&0.336	&0.932\\
& & dom & 0.393 &\best{0.430}&\best{0.479}&\best{0.531}&\best{0.201}&0.331&\best{0.366}&\best{0.561}&0.201&\best{0.236}&\best{0.281}&0.351&0.097&\best{0.176}&\best{0.331}&\best{0.895} \\
\cdashline{2-18}
& \multirow{2}{*}{Rnd} 
& full & 0.388 & 0.429 & \best{0.462} & \best{0.571} & 0.184 & 0.303 & 0.383 & 0.626 & 0.184 & 0.242 & 0.285 & 0.352 & 0.092 & 0.179 & 0.355 & \best{0.915} \\
& & dom & \best{0.381} & \best{0.423} & 0.476 & 0.670 & \best{0.183} & \best{0.284} & \best{0.367} & \best{0.614} & \best{0.182} & \best{0.233} & \best{0.282} & \best{0.349} & \best{0.087} & \best{0.170} & \best{0.323} & 1.020 \\
\cdashline{2-18}
& \multirow{2}{*}{Shuf} 
& full & 0.385 & 0.427 &  0.466 &  0.604 & 0.184 & 0.293 & 0.375  & 0.594 & 0.182 & 0.239 & 0.280 & 0.348 & 0.090 & 0.178 & 0.343 & 0.903 \\
& & dom & \best{0.373} & \best{0.421} & \best{0.452} & \best{0.510} & \best{0.174} & \best{0.263} & \best{0.348} & \best{0.502} & \best{0.179} & \best{0.232} & \best{0.275} & \best{0.342} & \best{0.084} & \best{0.169} & \best{0.303} & \best{0.750} \\
\hline
\multirow{8}{*}{\rotatebox{90}{Lightts~\cite{zhang2022less}}} & \multirow{2}{*}{Msk} 
& full & \best{0.418} & 0.432 & \best{0.573} & 0.621 & 0.204 & \best{0.238} & 0.321 & 0.435 & 0.163 & 0.206 & 0.258 & \best{0.317} &\best{0.096} & 0.388 & 0.518 & \best{0.774}\\
& & dom & \best{0.418} & \best{0.424} & 0.579 & \best{0.618} & \best{0.198} & 0.240 & \best{0.312} & \best{0.430} & \best{0.162} & \best{0.201} & \best{0.250} & \best{0.317} & 0.117 & \best{0.301} & \best{0.411} & 0.909\\
\cdashline{2-18}
& \multirow{2}{*}{Nois} & full & 0.445	&\best{0.442}&	0.590 &	0.654&
0.232	&\best{0.227}	&\best{0.342}	&0.446&
0.172	&0.223	&\best{0.259}	&0.324&	\best{0.092}	&0.279&	\best{0.451}&	\best{0.796}\\
& & dom &  \best{0.432}&0.451&\best{0.566}&\best{0.636}&\best{0.221}&0.236&0.351&\best{0.433}&\best{0.169}&\best{0.219}&\best{0.259}&\best{0.321}&0.095&\best{0.266}&0.488&0.820\\
\cdashline{2-18}
& \multirow{2}{*}{Rnd} 
& full & 0.419 & 0.436 & 0.647 & 0.713 & \best{0.205} & \best{0.244} & 0.360 & 0.494 & \best{0.164} & \best{0.213} & 0.267 & 0.329 & 0.097 & \best{0.281} & 0.524 & \best{0.852}  \\
& & dom & \best{0.414} & \best{0.431} & \best{0.570} & \best{0.610} & 0.206 & \best{0.244} & \best{0.324} & \best{0.442} & 0.171 & \best{0.213} & \best{0.263} & \best{0.323} & \best{0.096} & 0.299 & \best{0.422} & 1.222\\
\cdashline{2-18}
& \multirow{2}{*}{Shuf} 
& full & 0.415 & 0.426 & 0.577 & 0.621 & 0.202 & \best{0.235} & 0.325 & 0.445 & \best{0.163} & \best{0.205} & 0.251 & 0.317 & 0.096 & 0.367 & 0.535 & 1.420 \\
& & dom & \best{0.405} & \best{0.423} & \best{0.565} & \best{0.603} & \best{0.195} & 0.245 & \best{0.312} & \best{0.422} & 0.165 & \best{0.205} & \best{0.249} & \best{0.312} & \best{0.088} & \best{0.243} & \best{0.361} & \best{0.676}


==> tables/error_bars_ETT.tex <==
\begin{table}[!htb]
    \centering
    \addtolength{\tabcolsep}{-0.3em}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c@{\hspace{0.2em}}c|cccc|cc cc|cccc|cccc}
        \Xhline{2\arrayrulewidth}
        \multirow{2}{*}{Model} &   & \multicolumn{4}{c}{ETTh1} & \multicolumn{4}{c}{ETTh2} & \multicolumn{4}{c}{ETTm1} & \multicolumn{4}{c}{ETTm2} \\
        & & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 \\
        \hline
        \multirow{4}{*}{\makecell{iTrans \\former}} & Baseline& \base{0.391$\pm$0.001} & \base{0.448$\pm$0.002} & \base{0.483$\pm$0.003} & \base{0.515$\pm$0.003} & \base{0.302$\pm$0.001} & \base{0.381$\pm$0.000} & \base{0.413$\pm$0.001} & \base{0.432$\pm$0.002} & \base{0.342$\pm$0.002} & \base{0.386$\pm$0.003} & \base{0.421$\pm$0.001} & \base{0.491$\pm$0.003} & \base{0.184$\pm$0.001} & \base{0.253$\pm$0.002} & \base{0.312$\pm$0.001} & \base{0.411$\pm$0.001}  \\
        & Mask & 0.389$\pm$0.001 & 0.443$\pm$0.002 & 0.475$\pm$0.001 & 0.500$\pm$0.003 & 0.300$\pm$0.001 & 0.382$\pm$0.003 & 0.415$\pm$0.001 & 0.433$\pm$0.005 & 0.345$\pm$0.002 & 0.386$\pm$0.005 & 0.421$\pm$0.001 & 0.490$\pm$0.004 & 0.182$\pm$0.003 & 0.252$\pm$0.001 & 0.312$\pm$0.001 & 0.413$\pm$0.002 \\
        & Mix & 0.387$\pm$0.002 & 0.443$\pm$0.002 & 0.475$\pm$0.000 & 0.499$\pm$0.004 & 0.300$\pm$0.001 & 0.379$\pm$0.001 & 0.414$\pm$0.001 & 0.432$\pm$0.003 & 0.334$\pm$0.005 & 0.377$\pm$0.002 & 0.421$\pm$0.000 & 0.486$\pm$0.002 & 0.180$\pm$0.002 & 0.249$\pm$0.001 & 0.311$\pm$0.000 & 0.409$\pm$0.002\\
        & Ours& \best{0.383$\pm$0.001} & \best{0.439$\pm$0.001} & \best{0.472$\pm$0.002} & \best{0.494$\pm$0.002} & \best{0.296$\pm$0.002} & \best{0.378$\pm$0.003} &0.414$\pm$0.004 & 0.429$\pm$0.001 & \best{0.330$\pm$0.001} & \best{0.375$\pm$0.001} & \best{0.424$\pm$0.001} & \best{0.492$\pm$0.002} & \best{0.180$\pm$0.002} & \best{0.246$\pm$0.001} & \best{0.309$\pm$0.001} & \best{0.409$\pm$0.000}  \\
        \hline
        \Xhline{2\arrayrulewidth}
    \end{tabular}
    }
\end{table}

==> tables/error_bars_other4.tex <==
\begin{table}[!htb]
    \centering
    \addtolength{\tabcolsep}{-0.3em}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c@{\hspace{0.2em}}c|cccc|cc cc|cccc|cccc}
        \Xhline{2\arrayrulewidth}
        \multirow{2}{*}{Model} &   & \multicolumn{4}{c}{Electricity} & \multicolumn{4}{c}{Traffic} & \multicolumn{4}{c}{Weather} & \multicolumn{4}{c}{Exchange Rate} \\
        & & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 \\
        \hline
        \multirow{4}{*}{\makecell{iTrans \\former}} & Baseline& \base{0.151$\pm$0.000} & \base{0.157$\pm$0.001} & \base{0.176$\pm$0.003} & \base{0.217$\pm$0.013} & \base{0.399$\pm$0.001} & \base{0.418$\pm$0.000} & \base{0.429$\pm$0.000} & \base{0.463$\pm$0.000} & \base{0.174$\pm$0.001} & \base{0.225$\pm$0.001} & \base{0.281$\pm$0.000} & \base{0.359$\pm$0.003} & \base{\best{0.086$\pm$0.000}} & \base{0.180$\pm$0.000} & \base{0.337$\pm$0.002} & \base{0.860$\pm$0.004}  \\
        & Mask & 0.152$\pm$0.001 & 0.156$\pm$0.001 & 0.173$\pm$0.001 & 0.203$\pm$0.005 & 0.395$\pm$0.001 & \best{0.406$\pm$0.005} & \best{0.420$\pm$0.001} & 0.449$\pm$0.002 & 0.177$\pm$0.001 & 0.227$\pm$0.002 & 0.282$\pm$0.002 & 0.358$\pm$0.001 & 0.089$\pm$0.002 & 0.179$\pm$0.001 & 0.336$\pm$0.006 & 0.855$\pm$0.008 \\
        & Mix & 0.151$\pm$0.000 & 0.157$\pm$0.001 & 0.173$\pm$0.000 & 0.202$\pm$0.003 & 0.397$\pm$0.003 & 0.408$\pm$0.004 & 0.422$\pm$0.002 & 0.450$\pm$0.003 & 0.174$\pm$0.001 & 0.223$\pm$0.000 & 0.279$\pm$0.000 & 0.354$\pm$0.000 & 0.088$\pm$0.001 & 0.179$\pm$0.001 & 0.336$\pm$0.006 & 0.860$\pm$0.008\\
        & Ours& \best{0.150$\pm$0.000} & \best{0.155$\pm$0.001} & \best{0.171$\pm$0.000} & \best{0.196$\pm$0.002} & \best{0.394$\pm$0.000} & 0.411$\pm$0.002 & 0.421$\pm$0.002 & \best{0.448$\pm$0.001} & \best{0.171$\pm$0.001} & \best{0.221$\pm$0.000} & \best{0.276$\pm$0.000} & \best{0.352$\pm$0.002} & \best{0.085$\pm$0.001} & \best{0.177$\pm$0.001} & \best{0.320$\pm$0.006} & \best{0.821$\pm$0.003}\\
        \hline
        \Xhline{2\arrayrulewidth}
    \end{tabular}
    }
\end{table}

==> tables/long_term_3models_eth.tex <==

\multirow{11}{*}{\makecell{iTrans \\former \\ ~\cite{liu2024itransformer}}} & Baseline & \base{0.392} & \base{0.447} & \base{0.483} & \base{0.516} & \base{0.303} & \base{0.381} & \base{0.412} & \base{0.434} & \base{0.344} & \base{0.383} & \base{0.421} & \base{0.494} \\%& \base{0.183} & \base{0.251} & \base{0.311} & \base{0.412}  \\
& ASD~\cite{forestier2017generating} & 0.398 &0.456 &0.483 &0.512 &0.310 &0.388 &0.432 &0.452 &0.340 &0.382 &0.454&0.492\\
& MSB~\cite{bandara2021improving} &0.387&0.460&0.494&0.531&0.309&0.382&0.447&0.433&0.339&0.386&0.467&0.510\\
& Upsample~\cite{semenoglou2023data} & 0.391& 0.445&0.481&0.519&0.305&0.381&0.419&0.430&0.351&0.381&0.432&0.489\\
& FreqAdd~\cite{zhang2022self} & 0.389 & 0.446 & 0.475 & 0.510 & 0.300 & 0.384 & 0.416 & 0.438 & 0.350 & 0.385 & 0.422 & 0.490\\
& FreqPool~\cite{chen2023supervised} &0.433&0.456&0.497&0.549&0.324&0.397&0.402&0.479&0.354&0.390&0.423&0.498\\
& Robusttad~\cite{gao2020robusttad} &0.390&0.446&0.479&0.518&0.313&0.384&0.420&0.439&0.347&0.379&0.420&0.488\\
& STAug~\cite{zhang2023towards} & 0.390 & 0.445 &0.489 & 0.511& 0.323 & 0.428 & 0.486 & 0.483 & 0.339  & 0.383 & 0.417 & 0.485 \\
& FreqMask~\cite{chen2023fraug} & 0.390 & 0.442 & 0.475 & 0.497 & 0.301 & 0.385 & 0.414 & 0.438 & 0.347 & 0.383 & \best{0.420} & 0.494 \\%& 0.184 & 0.255 & 0.318 & 0.416 \\
& FreqMix~\cite{chen2023fraug} & 0.388 & 0.440 & 0.477 & 0.504 & 0.301 & \best{0.380} & 0.414 & 0.434 & 0.334 & 0.375 & 0.421 & \best{0.485} \\%& \best{0.178} & 0.248 & 0.311 & \best{0.407}\\
& Ours& \best{0.383} & \best{0.438} & \best{0.473} & \best{0.492} & \best{0.298} & 0.382 & \best{0.411} & \best{0.428} & \best{0.332} & \best{0.374} & 0.424 & 0.492 \\%& \best{0.178} & \best{0.246} & \best{0.309} & 0.409\\
\hline
\multirow{11}{*}{\makecell{TiDE \\ ~\cite{das2023longterm}}} & Baseline& \base{0.401} & \base{0.434} & \base{0.521} & \base{0.558} & \base{0.304} & \base{0.350} & \base{0.331} & \base{0.399} & \base{0.311} & \base{0.340} & \base{0.366} & \base{0.420} \\%& 
& ASD &0.417&0.441&0.513&0.556&0.320&0.351&0.367&0.422&0.319&0.341&0.399&0.432\\
& MSB &0.422&0.476&0.529&0.579&0.331&0.379&0.334&0.401&0.302&0.356&0.382&0.451\\
& Upsample &0.431&0.452&0.533&0.604&0.346&0.372&0.350&0.456&0.324&0.339&0.378&0.463\\
& FreqAdd & 0.385 & 0.420 & 0.477 & 0.505 & 0.289 & 0.336 & 0.330 & 0.390 & 0.309 & 0.339 &0.365&0.417\\
& FreqPool &\\
& Robusttad &\\
& STAug & 0.515 & 0.535 & 0.521 & 0.558 & 0.390 & 0.437 & 0.403 & 0.508 & 0.310 & 0.337 & 0.364 & 0.417\\
& Mask & 0.387 & 0.422 & 0.479 & 0.507 & 0.290 & 0.337 & 0.331 & 0.391 & 0.300 & 0.331 & 0.367 & 0.418 \\%& \best{0.165} & 0.219 & \best{0.271} & 0.348 \\
& Mix & \best{0.385} & 0.420 & 0.478 & 0.507 & 0.289 & 0.339 & 0.330 & 0.391 & 0.299 & 0.332 & 0.367 & 0.416 \\%& \best{0.165} & 0.219 & \best{0.271} & \best{0.347} \\
& Ours& \best{0.385} & \best{0.414} & \best{0.467} & \best{0.498} & \best{0.283} & \best{0.332} & \best{0.324} & \best{0.388} & \best{0.297} & \best{0.328} & \best{0.365} & \best{0.412} \\%& \best{0.165} & \best{0.218} & \best{0.271} & 0.350 \\
\hline
\multirow{11}{*}{\makecell{SCINet \\ ~\cite{liu2022scinet}}} & Baseline& \base{0.485} & \base{0.506} & \base{0.519} & \base{0.552} & \base{0.372} & \base{0.416} & \base{0.429} & \base{0.470} & \base{0.316} & \base{0.353} & \base{0.387} & \base{0.431} \\%& \base{0.184} & \base{0.240} & \base{0.295} & \base{0.385}  \\
& ASD &0.494&0.480&0.491&0.559&0.362&0.402&0.432&0.499&0.331&0.367&0.389&0.453\\
& MSB &0.489&0.466&0.502&0.547&0.359&0.396&0.458&0.476&0.320&0.351&0.396&0.478\\
& Upsample 0.471&0.457&0.479&0.541	&0.379&	0.407&	0.403&	0.482&	0.342&	0.386&	0.399	&0.442\\
& FreqAdd & 0.428 & 0.452 & 0.469 & 0.532 & 0.335 & 0.385 & 0.403 & 0.447 & 0.304 & 0.338 &0.373&0.421\\
& FreqPool &\\
& Robusttad &\\
& STAug & 0.457 & 0.500 & 0.524 & 0.534 & 0.538 & 0.636 & 0.681 & 0.648 & 0.319 & 0.357 & 0.389 & 0.445\\
& Mask & 0.429 & 0.454 & 0.471 & 0.547 & 0.340 & 0.386 & 0.406 & 0.451 & 0.308 & 0.344 & 0.379 & 0.427 \\%& 0.178 & 0.234 & 0.289 & 0.379 \\
& Mix & 0.427 & 0.452 & 0.465 & 0.548 & \best{0.335} & 0.377 & 0.400 & 0.438 & \best{0.302} & 0.341 & 0.376 & 0.423 \\%& \best{0.174} & 0.230 & 0.289 & \best{0.368} \\
& Ours& \best{0.417} & \best{0.443} & \best{0.461} & \best{0.527} & \best{0.335} & \best{0.375} & \best{0.392} & \best{0.421} & \best{0.302} & \best{0.338} & \best{0.372} & \best{0.420} \\%& \best{0.174} & \best{0.228} & \best{0.283} & 0.372 \\

==> tables/long_term_3models_weather.tex <==
% long-term 3 models weather datasets

        \multirow{2}{*}{Model} &   & \multicolumn{4}{c}{Electricity} & \multicolumn{4}{c}{Weather} & \multicolumn{4}{c}{Exchange Rate} \\
        & & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 \\
        \hline
        \multirow{11}{*}{\makecell{Auto \\former}} & Baseline& \base{0.203} & \base{0.208} & \base{0.231} & \base{0.239} & \base{0.241} & \base{0.314} & \base{0.341} & \base{0.425} & \base{0.143} & \base{0.305} & \base{0.470} & \base{1.056}  \\
        & ASD~\cite{forestier2017generating} &\\
        & MSB~\cite{bandara2021improving} &\\
        & Upsample~\cite{semenoglou2023data} &\\
        & FreqAdd~\cite{zhang2022self} & 0.193 & 0.197 & 0.212 & 0.225 & 0.255 & 0.323 & 0.370 & 0.419 & 0.143 & 0.369 & 0.716 & 1.173 \\
        & FreqPool~\cite{chen2023supervised} &\\
        & Robusttad~\cite{gao2020robusttad} &\\
        & STAug~\cite{zhang2023towards} & 0.191 & 0.206 & 0.217 & 0.234 & 0.250 & 0.300 & 0.347 & 0.418 & 0.140 & 0.326 & 0.594 & 1.176\\
        & Mask~\cite{chen2023fraug} & 0.180 & 0.197 & 0.210 & 0.224  & 0.245 & 0.290 & 0.340 & 0.392 & 0.142 & 0.410 & 0.471 & 0.778 \\
        & Mix~\cite{chen2023fraug} & 0.177 & 0.194 & 0.206 & 0.228 & 0.240 & 0.302 & 0.330 & 0.422 & 0.141 & 0.284 & 0.453 & 0.834 \\
        & Ours& \best{0.171} & \best{0.191} & \best{0.203} & \best{0.219}  & \best{0.214} & \best{0.273} & \best{0.327} & \best{0.383} & \best{0.136} & \best{0.243} & \best{0.418} & \best{0.695} \\
        \hline
        \multirow{11}{*}{MICN} & Baseline& \base{0.171} & \base{0.183} & \base{0.198} & \base{0.224} & \base{0.188} & \base{0.241} & \base{0.278} & \base{0.350} & \base{0.091} & \base{0.185} & \base{0.355} & \base{0.941}  \\
        & ASD &0.165	&0.174&	0.19	&0.237&0.189&	0.242	&0.276&	0.354	&0.087	&0.175 	&0.337	&1.203\\
        & MSB &0.179	&0.182&	0.201	&0.225&0.201&	0.250 &	0.291&	0.365&	0.088	&0.176&	0.360 &	0.995\\
        & Upsample &0.182	&0.180 &	0.203	&0.220 &0.193	&0.249	&0.279&	0.372	&0.084&	0.171	&0.303	&0.702\\
        & FreqAdd & 0.160 & 0.169 & 0.182 & 0.199 & 0.180 & 0.234 & 0.282 & 0.350 & 0.087 & 0.174 & 0.349 & 0.923 \\
        & FreqPool &\\
        & Robusttad &\\
        & STAug & 0.180 & 0.195 & 0.210 & 0.224 & 0.272 & 0.356 & 0.433 & 0.559 & 0.092 & 0.183 & 0.313 & 0.790 \\
        & Mask & 0.159 & 0.164 & 0.180 & 0.200 & 0.190 & 0.236 & 0.281 & 0.345 & 0.085 & 0.173 & 0.339 & 0.847 \\
        & Mix & 0.159 & 0.165 & 0.178 & 0.195 & 0.185 & 0.239 & 0.281 & 0.344 & 0.086 & 0.174 & 0.337 & 0.796 \\
        & Ours& 0.157 & 0.168 & 0.178 & 0.211 & 0.179 & 0.232 & 0.275 & 0.342 & 0.084 & 0.169 & 0.303 & 0.750 \\
        \hline
        \multirow{11}{*}{Lightts} & Baseline& \base{0.210} & \base{0.169} & \base{0.182} & \base{0.212} & \base{0.168} & \base{0.210} & \base{0.260} & \base{0.320} & \base{0.139} & \base{0.252} & \base{0.412} & \base{0.840}  \\
        & ASD &0.225	&0.179	&0.198&	0.232&0.179	&0.21	&0.271&	0.321&	0.132	&0.320 &	0.436&	1.036\\
        & MSB &0.233	&0.182	&0.204	&0.228&0.17	&0.214&	0.259	&0.332&	0.117&	0.294	&0.502	&0.964\\
        & Upsample &0.246 &	0.179	 &0.211 &	0.254 &0.182	 &0.223	 &0.257	 &0.336	 &0.099 &	0.251 &	0.369	 &0.702\\
        & FreqAdd & 0.213 & 0.157 & 0.177 & 0.206 & 0.164 & 0.207 & 0.258 & 0.317 & 0.098 & 0.522 & 0.565 & 1.583\\
        & FreqPool &\\
        & Robusttad &\\
        & STAug & 0.224 & 0.267 & 0.294 & 0.351 & 0.214 & 0.263 & 0.382 & 0.371 & 0.096 & 0.522 & 
        0.565 & 1.583 \\
        & Mask & 0.200 & 0.157 & 0.175 & 0.206  & 0.163 & 0.206 & 0.258 & 0.317 & 0.096 & 0.388 & 0.518 & 0.774 \\
        & Mix & 0.192 & 0.158 & 0.175 & 0.211 & 0.165 & 0.206 & 0.257 & 0.318 & 0.099 & 0.384 & 0.540 & 1.278 \\
        & Ours& 0.210 & 0.156 & 0.173 & 0.206 & 0.165 & 0.205 & 0.249 & 0.312 & 0.088 & 0.243 & 0.361 & 0.676

